MM1.5: Methods, Analysis & Insights from Multimodal LLM Fine-tuning

We present MM1.5, a new family of multimodal large language models (MLLMs) designed to enhance capabilities in text-rich image understanding, visual referring and grounding, and multi-image reasoning. Building upon the MM1 architecture, MM1.5 adopts a data-centric approach to model training, systematically exploring the impact of diverse data mixtures across the entire model training lifecycle. This includes high-quality OCR data and synthetic captions for continual pre-training, as well as an optimized visual instruction-tuning data mixture for supervised fine-tuning. Our models range from 1B to 30B parameters, encompassing both dense and mixture-of-experts (MoE) variants, and demonstrate that careful data curation and training strategies can yield strong performance even at small scales (1B and 3B). Additionally, we introduce two specialized variants: MM1.5-Video, designed for video understanding, and MM1.5-UI, tailored for mobile UI understanding. Through extensive empirical studies and ablations, we provide detailed insights into the training processes and decisions that inform our final designs, offering valuable guidance for future research in MLLM development.

==> figs/alpha_ablation/combined.tex <==
\begin{figure*}%[ht!]
\centering
\begin{subfigure}[b]{0.49\textwidth}
    \input{figs/alpha_ablation/alpha_a}
    \vspace{0.36cm}
    \caption{Science Mixture}
\end{subfigure} \hfill
\begin{subfigure}[b]{0.49\textwidth}
    \input{figs/alpha_ablation/alpha_b}
    \vspace{0.36cm}
    \caption{Math Mixture}
\end{subfigure} \\
\begin{subfigure}[b]{0.49\textwidth}
    \input{figs/alpha_ablation/alpha_c}
    \vspace{0.78cm}
    \caption{Code Mixture}
\end{subfigure} \hfill
\begin{subfigure}[b]{0.49\textwidth}
    \input{figs/alpha_ablation/alpha_d}
    \vspace{0.36cm}
    \caption{Refer/Ground Mixture}
\end{subfigure}
    \caption{Impact of $\alpha$ for different data categories to a model's main capabilities. The selected ratio is marked with red ``x''.}
    \label{fig:ratio_impact_single}
%\vspace{-2mm}
\end{figure*}

==> figs/latex_examples/nyt.tex <==
{
\renewcommand{\arraystretch}{0.0}
\begin{tabular}{@{}l@{}}
\begin{topbox}

        \begin{center}\includegraphics[width=0.6\textwidth]
        {figs/examples/NYTimes-Page1-11-11-1918.jpg} \end{center}\\
         Could you summarize every article on this newspaper page? \zhe{Sam: check that this is from 3b model}
\end{topbox}\\
\begin{bottombox}
    The newspaper page is from The New York Times dated November 11, 1918. The main headline announces the signing of the Armistice, marking the end of World War I. Other articles cover the revolution in Germany, with Berlin being seized by revolutionists and the abdication of Kaiser Wilhelm II. The page also includes a call for the abdication of the German Emperor by the socialist Chancellor, Friedrich Ebert. Additionally, there are reports on the ousting of Kaiser Wilhelm II and his flight to the Netherlands, as well as the resignation of the German General Staff. The page also features a report on the armistice being signed in France, marking the end of the war.
\end{bottombox}
\end{tabular}%
}

==> figs/latex_examples/wikitable.tex <==
{
\renewcommand{\arraystretch}{0.0}
\begin{tabular}{@{}l@{}}
\begin{topbox}

        \begin{center}\includegraphics[width=0.6\textwidth]
        {figs/examples/wikitable.png} \end{center}\\
         Can you give me a table of the countries in this list and the gdp, but only give me countries from asia \zhe{Sam: check that this is from 3b model}
\end{topbox}\\
\begin{bottombox}
    Sure, here is a table of the Asian countries in the list and their forecasted GDP in 2024:Country/TerritoryForecastChina18,532,633Japan4,110,452India3,937,011South Korea1,760,947Indonesia1,475,690Thailand548,890Philippines471,516Vietnam465,814Iran464,181Bangladesh455,162Malaysia445,519Hong Kong406,775Singapore525,228Note: The GDP figures are in billions of US dollars.
\end{bottombox}
\end{tabular}%
}

==> figs/sft_mixture/table3.tex <==
\begin{tabular}{llllll}
        \toprule
        \cellcolor{Cerulean!60} \textbf{General} & \cellcolor{Goldenrod!60} \textbf{Text Rich} & \cellcolor{Orange!60} \textbf{Knowledge (Math/Science/Code)} & \cellcolor{Purple!60} \textbf{Referring \& Grounding} &  \cellcolor{Green!60} \textbf{Multi-image} & \cellcolor{red!60} \textbf{Text} \\

\end{tabular}

==> tables/benchmark_categories.tex <==
\begin{table}[h!]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c}
    \toprule
         Capability& Benchmarks\\
         \midrule
         General& MME~\cite{fu2024mmecomprehensiveevaluationbenchmark}, SeedBench~\cite{li2023seedbenchbenchmarkingmultimodalllms}, POPE~\cite{li2023evaluating}, LLaVA-Bench$^\text{W}$~\cite{llava}, MM-Vet~\cite{yu2023mmvetevaluatinglargemultimodal}, RealworldQA~\cite{grok15v}\\
         Text-rich& WTQ~\cite{pasupat2015compositional}, TabFact~\cite{chen2019tabfact}, OCRBench~\cite{liu2024hiddenmysteryocrlarge}, ChartQA~\cite{masry2022chartqa}, TextVQA~\cite{singh2019towards}, DocVQA~\cite{mathew2021docvqa}, InfoVQA~\cite{mathew2022infographicvqa}\\
         Refer\&Ground& Flickr30k~\cite{young2014image}, LVIS-Ref~\cite{you2023ferret}, RefCOCO~\cite{kazemzadeh2014referitgame}, RefCOCOg, RefCOCO+\\
         Knowledge& AI2D~\cite{kembhavi2016diagram}, ScienceQA~\cite{lu2022learn}, MathVista~\cite{lu2023mathvista}, MMMU~\cite{yue2023mmmu}\\
         Multi-image & Q-Bench2~\cite{zhang2024benchmark}, Mantis~\cite{jiang2024mantis}, NLVR2~\cite{suhr2018corpus}, BLINK~\cite{fu2024blink}, MVBench~\cite{li2023mvbench} \\
         \bottomrule
    \end{tabular}
    }
    \vspace{1mm}
    \caption{Benchmark groups based on different capabilities for ablation study.}
    \label{tab:benchmark_category}
\end{table}
